Optimal Matrix-Mimetic Tensor Algebras via Variable Projection

Recent advances in {matrix-mimetic} tensor frameworks have made it possible to preserve linear algebraic properties for multilinear data analysis and, as a result, to obtain optimal representations of multiway data. Matrix mimeticity arises from interpreting tensors as operators that can be multiplied, factorized, and analyzed analogous to matrices. Underlying the tensor operation is an algebraic framework parameterized by an invertible linear transformation. The choice of linear mapping is crucial to representation quality and, in practice, is made heuristically based on expected correlations in the data. However, in many cases, these correlations are unknown and common heuristics lead to suboptimal performance. In this work, we simultaneously learn optimal linear mappings and corresponding tensor representations without relying on prior knowledge of the data. Our new framework explicitly captures the coupling between the transformation and representation using variable projection. We preserve the invertibility of the linear mapping by learning orthogonal transformations with Riemannian optimization. We provide original theory of uniqueness of the transformation and convergence analysis of our variable-projection-based algorithm. We demonstrate the generality of our framework through numerical experiments on a wide range of applications, including financial index tracking, image compression, and reduced order modeling. We have published all the code related to this work at https://github.com/elizabethnewman/star-M-opt.

==> sections/S_02_01_tsvdm_derivatives.tex <==
\subsection{Derivative of Truncated Matrix SVD}
\label{app:truncatedSVDDerivation}

\def\dU{\magenta{\delta \bfU}}
\def\dS{\cyan{\delta \bfSigma}}
\def\dV{\orange{\delta \bfV}}
\def\dA{\blue{\delta \bfA}}

The goal of this section is to compute the derivatives through the truncated SVD of a matrix $\bfA \in \Rbb^{n_1\times n_2}$.   
The presented derivation is based on various resources including~\cite{Townsend2016, Giles1948, Wan2019:complexSVD, minka1997old}.  
Let $r = \min(n_1,n_2)$ and let $\bfA = \bfU \bfSigma \bfV^\top$ be the economic SVD where $\bfU \in \Rbb^{n_1\times r}$ and $\bfV\in \Rbb^{n_2\times r}$ have orthonormal columns and $\bfSigma\in \Rbb^{r\times r}$ is a diagonal matrix with real, nonnegative diagonal entries in decreasing order.  
Our goal is to compute the following derivatives:
	\begin{subequations}
	\begin{alignat}{3}
	&\nabla_{\bfA} \bfU &&:  \Rbb^{n_1\times r} &&\to \Rbb^{n_1\times n_2}\\
	&\nabla_{\bfA} \bfSigma &&: \Rbb^{r\times r} &&\to \Rbb^{n_1\times n_2}\\
	&\nabla_{\bfA} \bfV &&: \Rbb^{n_2\times r} &&\to \Rbb^{n_1\times n_2}
	\end{alignat}
	\end{subequations}
The formulas we ultimately obtain are the following:
	\begin{subequations}
	\begin{align}
	\nabla_{\bfA} \bfU(\dU) &=[\bfU (\bfF \odot (\bfU^\top \dU - \dU^\top \bfU)) \bfSigma + (\bfI_{n_1} - \bfU \bfU^\top) \dU \bfSigma^{-1}] \bfV^\top\\
	\nabla_{\bfA} \bfSigma_k(\dS) &= \bfU(\bfI_r \odot \dS) \bfV^\top\\
	\nabla_{\bfA} \bfV(\dV) &= \bfU [\bfSigma (\bfF \odot (\bfV^\top\dV- \dV^\top \bfV) \bfV^\top + \bfSigma^{-1}\dV (\bfI_{n_2} - \bfV\bfV^\top)]
	\end{align}
	\end{subequations}

Without loss of generality, assume $n_1 \le n_2$.   
We can use a similar  derivation for $n_2 > n_1$ applied to $\bfA^\top$. 
%Given matrix SVD $\bfA = \bfU \bfSigma \bfV^\top$, let $\bfSigma\in \Rbb^{n_1\times n_1}$ be a diagonal matrix and  let $\bfV = \begin{bmatrix}\bfV & \bfV_2 \end{bmatrix}$ be the full right singular matrix partitioned into $\bfV \in \Rbb^{n_2\times n_1}$ and $\bfV_2 \in \Rbb^{n_2\times n_2-n_1}$
If we perturb the factor matrices by a small amount, e.g., $\bfU + \varepsilon\dU$ where $\varepsilon>0$ is small, the matrix $\bfA$ and the orthogonality constraints are perturbed accordingly via
	\begin{align}
	\begin{split}
	\bfA + \varepsilon\dA+ \Ocal(\varepsilon^2) 
		&= (\bfU + \varepsilon\dU)(\bfSigma + \varepsilon\dS)(\bfV + \varepsilon\dV^\top)\\
		&=\bfU\bfSigma\bfV^\top +\varepsilon\left( \dU \bfSigma \bfV^\top + \bfU \dS \bfV^\top + \bfU \bfSigma \dV^\top\right) + \Ocal(\varepsilon^2).
	\end{split}
	\end{align}

We additionally require that the perturbations of the factor matrices do not change the structure of the SVD; that is, $\dS$ is a diagonal matrix and the perturbations of the left and right singular matrices satisfy the orthogonality constraints
	\begin{align}
	 \bfI_{n_1} &=(\bfU + \varepsilon \dU)^\top (\bfU + \varepsilon \dU) \\
	 				&=\bfU^\top \bfU + \varepsilon(\dU^\top \bfU + \bfU^\top \dU) + \varepsilon^2 \dU^\top \dU 
	\end{align}
A similar derivation can be performed for $\bfV$.  

Note that the constant terms cancel in the above equalities.  
Additionally, as $\varepsilon \downarrow 0$, the $\varepsilon^2$ terms become negligible, which results in the following relationships in differentials:
	\begin{subequations}\label{eqn:partials}
	\begin{align}
	\dA&= \dU \bfSigma \bfV^\top + \bfU \dS \bfV^\top + \bfU \bfSigma \dV^\top\label{eqn:dA}\\
	{\bf0}_{n_1} &= \dU^\top \bfU + \bfU^\top \dU\label{eqn:dU}\\
	{\bf0}_{n_1} &=\dV^\top \bfV + \bfV^\top \dV \label{eqn:dV}\\
	\dS &\text{ diagonal} \label{eqn:dS}
	\end{align}
	\end{subequations}
One key observation is that $\bfU^\top \dU$ and $\bfV^\top \dV$ are real-valued, antisymmetric matrices, and hence have zeros along the diagonal. 

We first solve for $\dS$ by multiplying~\eqref{eqn:dA} on the left and right by $\bfU^\top$ and  $\bfV$, respectively
	\begin{align}\label{eqn:UdAV}
	\bfU^\top \dA\bfV &= \bfU^\top \dU \bfSigma +  \dS + \bfSigma \dV^\top\bfV.
	\end{align}
Because $\bfU^\top \dU$ and $\bfV^\top \dV$ are antisymmetric and $\bfSigma$ and $\dS$ are diagonal matrices, the only nonzero diagonal entries occur in $\dS$.  
Hence, 
	\begin{align}
	\dS = \bfI_{n_1 \times n_1} \odot (\bfU^\top \dA\bfV)
	\end{align}
where $\odot$ denotes the Hadamard entrywise product. 
Next, we compute $\dU$ by first multiplying~\eqref{eqn:UdAV} on the right by $\bfSigma$ and transposing of both sides of the equality, resulting in the following system of equations
	\begin{align}
	\bfU^\top \dA\bfV\bfSigma &= \bfU^\top \dU \bfSigma^2 + \bfSigma \dV^\top\bfV \bfSigma \\
	\bfSigma \bfV^\top \dA^\top \bfU   &= -\bfSigma^2\bfU^\top \dU  - \bfSigma \dV^\top\bfV \bfSigma.
	\end{align}
We used the antisymmetry of $\bfU^\top \dU$ and ignored the contribution of $\dS$ because we only need to develop formulas for the off-diagonal entries.  
We add the two equations, and obtain the following equality:
	\begin{align}
	\bfU^\top \dA\bfV\bfSigma + \bfSigma \bfV^\top \dA^\top \bfU  &= \bfU^\top \dU \bfSigma^2  -\bfSigma^2\bfU^\top \dU
	\end{align}
Because $\bfSigma$ is a diagonal matrix, we can solve for $\bfU^\top \dU$ via
	\begin{align}
	\bfF \odot (\bfU^\top \dA\bfV \bfSigma +  \bfSigma \bfV^\top \dA^\top \bfU) &= \bfU^\top \dU
	\end{align}
where
	\begin{align}
	\bfF_{ij} = \begin{cases}
			\dfrac{1}{\sigma_j - \sigma_i},  & i\not= j\\
			0, &i = j.
			\end{cases}
	\end{align}
The final step is to solve for $\dU$.  
Using the orthogonality of $\bfU$, we get
	\begin{align}
	\dU = \bfU [\bfF \odot (\bfU^\top \dA\bfV\bfSigma +\bfSigma \bfV^\top \dA^\top \bfU )].
	\end{align}
We use a similar technique to solve for $\dV$, resulting in 
	\begin{align}
	\dV =  \bfV [\bfF \odot (\bfSigma\bfU^\top \dA\bfV + \bfV^\top \dA^\top \bfU \bfSigma)].
	\end{align}

The formulas above are forward mode derivatives (i.e., how changes in $\bfA$ lead to changes in the factors).  
We are interested in reverse mode derivatives (i.e., how changes in the factors lead to changes in the $\bfA$). 

In our current implementation, we compute the derivative of the full SVD and zero out the directions pertaining to the small singular values. 
This seemed to give more robust performance in our algorithm than the direct low-rank versions of the derivatives. 
We will focus on low-rank implementations in future versions of the code as part of the push to improve efficiency.


